Synthesizing Stealthy Reprogramming Attacks on Cardiac Devices

An Implantable Cardioverter Defibrillator (ICD) is a medical device used for the detection of potentially fatal cardiac arrhythmia and their treatment through the delivery of electrical shocks intended to restore normal heart rhythm. An ICD reprogramming attack seeks to alter the device's parameters to induce unnecessary shocks and, even more egregious, prevent required therapy. In this paper, we present a formal approach for the synthesis of ICD reprogramming attacks that are both effective, i.e., lead to fundamental changes in the required therapy, and stealthy, i.e., involve minimal changes to the nominal ICD parameters. We focus on the discrimination algorithm underlying Boston Scientific devices (one of the principal ICD manufacturers) and formulate the synthesis problem as one of multi-objective optimization. Our solution technique is based on an Optimization Modulo Theories encoding of the problem and allows us to derive device parameters that are optimal with respect to the effectiveness-stealthiness tradeoff (i.e., lie along the corresponding Pareto front). To the best of our knowledge, our work is the first to derive systematic ICD reprogramming attacks designed to maximize therapy disruption while minimizing detection. To evaluate our technique, we employ an extensive dataset of synthetic EGMs (cardiac signals), each generated with a prescribed arrhythmia, allowing us to synthesize attacks tailored to the victim's cardiac condition. Our approach readily generalizes to unseen signals, representing the unknown EGM of the victim patient.

==> trans_encoding.tex <==
\subsection{Discrimination Algorithms as Symbolic Transducers}
We formalize the behavior of the BS and Medtronic discrimination algorithms as \textit{symbolic finite transducers (SFTs)}~\cite{veanes2012symbolic,d2017power}. We first provide some background on this formal model. Classical finite transducers extend finite automata in that they map input strings into output strings, while classical automata can only recognize a given string, i.e., establish if the string belongs to the underlying language. SFTs are a powerful extension of classical transducers where transitions can be labeled with arbitrary formulas from any decidable theory, leveraging state-of-the-art satisfiability modulo theory (SMT) solvers to provide such decision procedures. In our study, we use SFTs to describe the mapping of cardiac signals into the corresponding therapy signals.

For instance, classical transducers have transitions of the form $q \goes{a / b} q'$, i.e. that read from state $q$ a symbol $a$ and produces an output $b$ before moving to state $q'$. Their symbolic counterpart are extremely more expressive and have transitions of the form $q \goes{\gamma / v} q'$, i.e., that read from state $q$ a symbol $a$ that satisfies predicate $\gamma$ and, before moving to $q'$, produce in output a sequence of symbols obtained by applying function $v$ to $a$.

We follow the presentation of SFTs of~\cite{veanes2012symbolic}. Since SFTs are labeled with predicates, we consider a \textit{background structure} with multi-typed domain $\mathcal{U}$ and fixed interpretation for function and relation symbols. For type $\tau$, we denote with $\mathcal{U}^\tau$ the sub-domain of elements of type $\tau$. We denote with $\sigma$ the type of \textit{input elements}, with domain $\Sigma = \mathcal{U}^\sigma$, and $\gamma$ the type of \textit{output elements}, with domain $\Gamma = \mathcal{U}^\gamma$. The Boolean type is $\mathbb{B}$, with $\mathcal{U}^{\mathbb{B}} = \{ \bot, \top \}$. Terms and formulas are defined by induction over the background language and are assumed to be well-typed. We assume that each element of $\mathcal{U}$ has a corresponding constant symbol in the background language. A term $t$ of type $\tau$ is denoted as $t : \tau$ and its set of free variables as $FV(t)$. Given a closed term $t : \tau$ (i.e., where $FV(t) = \emptyset$), let $[\![t]\!] \in \mathcal{U}^\tau$ denote its interpretation.

A $\lambda$-term $f$ describes a function from input elements to output elements. Technically $f$ is an expression of the form $\lambda x.t$, where $x : \sigma$ is an input variable and $t : \gamma$ is an output term with at most one free variable for the input symbol ($FV(t) \subseteq \{ x \}$). The type of $f$ is $\sigma \rightarrow \gamma$ and its interpretation is the function $[\![f]\!] : \Sigma \rightarrow \Gamma$ mapping $a \in \Sigma$ to $[\![t[x/a]]\!]$, where $t[x/a]$ is the term obtained by substituting $x$ with $a$ in $t$. A $\lambda$-term of type $\sigma \rightarrow \mathbb{B}$ is called $\sigma$-predicate. For $\sigma$-predicate $\varphi$ and $a \in \Sigma$, we write $a \in [\![\varphi]\!]$ for $[\![\varphi]\!](a) = \top$. In other words, $[\![\varphi]\!]$ is the set of input elements that satisfy predicate $\varphi$. A \textit{label theory} for $\sigma \rightarrow \gamma$ consists of a set of $\lambda$-terms of type $\sigma \rightarrow \gamma$ and a set of $\sigma$-predicates closed under Boolean operations. We focus on \textit{decidable} theories, i.e., where checking satisfiability of a predicate $\varphi$ (whether or not $[\![\varphi]\!] \neq \emptyset$) is decidable.


\begin{example}\label{xmpl:SFT_1}
An example of decidable label theory for $\mathbb{R} \rightarrow \mathbb{B}$ is the theory of quantifier-free linear real arithmetic. In our context, an example $\mathbb{R}$-predicate is 
$$\mathsf{VFstart}(x) \overset{\bf def}{=} \left( \sum_{n=0}^9 \mathsf{ite}(\mathsf{Vperiod}(x-n)<\mathrm{VF_{th}},1,0) \right) \geq 8$$
where $x$ is a free variable denoting the number of ventricular beats occurred since the beginning of the signal, $\mathsf{ite}$ is the if-then-else function, and $\mathsf{Vperiod}(x)$ is the macro 
$\mathsf{ite}\left( x \leq 1,   \mathsf{Vperiod}_1, \mathsf{ite}\left( x = 2,   \mathsf{Vperiod}_2,  \mathsf{ite}\left( x = 3,   \mathsf{Vperiod}_3,  \ldots \right)  \right)  \right)$, where $\mathsf{Vperiod}_i$ is the constant denoting the ventricular period for the $i$-th cycle. We can see that predicate $\mathsf{VFstart}(x)$ encodes the first discriminator of the BS algorithm.
\end{example}

\begin{definition}
A \emph{symbolic finite transducer (SFT)} over $\sigma \rightarrow \gamma$ is a tuple $(Q,q_0,F,R)$ where $Q$ is a finite set of \emph{states}, $q_0 \in Q$ is the \emph{initial state}, $F \subseteq Q$ is the set of \emph{final states}, and $R$ is a set of rules of the form $(q,\varphi,\mathbf{f}, q')$, also denoted as $q\goes{\varphi/\mathbf{f}}q'$, where $q,q' \in Q$ are the \emph{source and target states}, $\varphi$ is a $\sigma$-predicate called \emph{guard}, and $\mathbf{f} = \lambda x . (\mathbf{f}[0](x), \ldots,  \mathbf{f}[k](x))$ is a sequence of $\lambda$-terms called the \emph{output} (with $k=|\mathbf{f}|$), over a given label theory for $\sigma \rightarrow \gamma$.
\end{definition}

A rule $q\goes{\varphi/\mathbf{f}}q'$ entails a number of concrete transitions, or \textit{instances}, $q\goes{a/\mathbf{b}}q'$, where $a \in [\![\varphi]\!]$ is an input symbol that satisfies the guard $\varphi$ and $\mathbf{b} = [\![\mathbf{f}]\!](a)$ is the sequence of elements obtained by applying the sequence of $\lambda$-terms $\mathbf{f}$ to $a$.

\begin{example}
Consider the predicate $\mathsf{VFstart}$ introduced in Example~\ref{xmpl:SFT_1}. An example SFT rule is $q \goes{\neg \mathsf{VFstart} / \bot} q$ that, from state $q$, accepts inputs (in this case the current number of ventricular beats) that satisfy $\neg \mathsf{VFstart}$ (i.e., do not satisfy the first BS discriminator) and outputs $\bot$, indicating that no therapy is given.
\end{example}

In the following definitions, we assume a fixed SFT $T = (Q,q_0,F,R)$.

\begin{definition}
For $\mathbf{a} \in \Sigma^*$, $\mathbf{b} \in \Gamma^*$, we denote with $q \goess{\mathbf{a}/\mathbf{b}} q'$ the \emph{reachability relation}, i.e., relating states $q$ that can reach states $q'$ with an input sequence $\mathbf{a}$ producing an output sequence $\mathbf{b}$:
$$q = q^0 \goes{\mathbf{a}[0]/\mathbf{b}^0} q^1 \ldots q^n \goes{\mathbf{a}[n]/\mathbf{b}^n} q^{n+1} = q',$$
where $n = |\mathbf{a}| - 1$ and $\mathbf{b}$ can be rewritten as the concatenation $\mathbf{b} = \mathbf{b}^0 \ldots \mathbf{b}^n$. For any $q \in Q$, $q \goess{\epsilon/\epsilon} q$, where $\epsilon$ is the empty symbol.
\end{definition}

We now define the transduction of $T$, which characterizes the set of admissible output sequences of $T$, i.e., those produced by any path from the initial state to a final state.

\begin{definition}
The transduction of $T$, $\mathcal{T}_T$, is the function mapping input sequences $\mathbf{a} \in \Sigma^*$ to the set
$$\mathcal{T}_T(\mathbf{a}) \overset{\bf def}{=} \{ \mathbf{b} \in \Gamma^* \mid \exists q \in F . \ q_0 \goess{\mathbf{a} / \mathbf{b}} q \}.$$
\end{definition}

The transducer $T$ is deterministic when, for any pair of rules $q\goes{\varphi/\mathbf{f}}q_1$ and $q\goes{\psi/\mathbf{g}}q_2$, if $\varphi$ and $\psi$ are not mutually exclusive ($[\![\varphi \wedge \psi]\!] \neq \emptyset$), then $q_1 = q_2$ and $\mathbf{f}$ and $\mathbf{g}$ are equivalent w.r.t.\ $\varphi \wedge \psi$, i.e., the predicate $\lambda x. \varphi(x) \wedge \psi(x) \wedge \mathbf{f}(x) \neq \mathbf{g}(x)$ is unsatisfiable. It follows that, when $T$ is deterministic, its transduction is \textit{1-valued}, i.e., $|\mathcal{T}_T(\mathbf{a})| \leq 1$ for any $a \in \Sigma^*$, and thus, $\mathcal{T}_T$ can be seen as a function from input sequences to output sequences. It is easy to verify that a sufficient condition for determinism is that all the guards out of the same state are mutually exclusive. 

For the encoding of the arrythmia discrimination algorithms, we consider an extension of SFTs with registers, i.e., where the states are represented symbolically by a set of variables, the registers. We omit here the formal definition (available in~\cite{veanes2012symbolic}), which is analogous to that of SFTs. In our encoding, we will keep the finite state component separate from the registers, and use extended rules of the form $q\goes{\varphi/\mathbf{f}; \ r \gets t}q'$ to denote that the value of register $r$ is updated to $t$ when stepping into $q'$. 

To simplify the presentation of our models, we extend the SFT notation with a set of \textit{hold states} $H$ ($H \cap Q = \emptyset$) that hold the previous input symbol once they are visited, instead of evaluating a new one. From this extension, a regular SFT can be readily obtained by iteratively replacing every pair of consecutive rules $q\goes{\varphi/\mathbf{f}} q' \goes{\varphi'/\mathbf{f}'} q''$ where $q \in Q$, $q' \in H$ and $q'' \in Q \cup H$, with the rule $q \goes{\varphi \wedge \varphi'/\mathbf{f}.\mathbf{f}'} q''$ until no hold state can be reached from the initial state, where $\mathbf{f}.\mathbf{f}'$ is the concatenation of $\mathbf{f}$ and $\mathbf{f}'$. However such an extension requires that, for any rule $q\goes{\varphi/\mathbf{f}} q'$ where $q \in H \vee q' \in H$, $FV(\mathbf{f}) = \emptyset$, i.e., the output is constant and does not depend on the input element.

\paragraph{SFT of BS algorithm.} We introduce the SFT model of the BS discrimination algorithm, depicted in Figure~\ref{fig:BS_SFT}. Since we are interested in analyzing the behavior of the algorithm offline over a fixed set of signals, we can effectively pre-compute for each signal the non-linear operations underlying some of the discriminators, such as the computation of the correlation scores between the shock EGM and the NSR template, or the ventricular period variances. This allows us to define an SFT over the decidable theory of quantifier-free real arithmetic. Importantly, we pre-compute only the operations that are not affected by the ICD parameters, meaning that our SFT formalization is suitable for the parametric analysis required to study the reprogramming attacks.

Thanks to this pre-processing, the inputs of the SFT are no longer sequences of atrial, ventricular and shock EGMs, but are sequences of the form $1,2,3\ldots$ describing the progressive number of heart cycles, i.e. of ventricular periods. In this way, we can drastically reduce the length of the input sequence, thus leading to a lower computational cost. As an example, a 1-minute EGM signal with a relatively low sampling rate of 1 kHz lead to an input sequence of length 6000. In contrast, the number of heart cycles depends on the HR, but produce much shorter sequences. The worst case is that of ventricular fibrillation where the HR can reach 500 BPM (input sequence of length 500). 

The transduction of this SFT gives the corresponding therapy signal, i.e., a Boolean sequence indicating, for each heart beat, whether or not therapy is delivered. ICD parameters are encoded as uninterpreted constants.

From the initial state $q_0$, if the predicate $\mathsf{VFstart}$ (defined in Example~\ref{xmpl:SFT_1}) is satisfied by the current input, the algorithm initiates the VF duration window and the SFT transitions into the state $\mathsf{VF_d}$, delivering no therapy for the moment. Similarly, if the start of VT is detected ($\neg \mathsf{VFstart} \wedge \mathsf{VTstart}$), the SFT moves to the state $\mathsf{VT_d}$ describing the VT duration window. Registers $\mathsf{t_{VF}}$ and $\mathsf{t_{VT}}$ keep track of the time spent in the VF and VT windows, respectively. If both $\mathsf{VFstart}$ and $\mathsf{VTstart}$ are false, we stay in $q_0$ with no therapy delivered. 


\begin{figure}
\newcommand{\thrp}{{\color{red!60!black} \top}}
\newcommand{\nthrp}{{\color{green!60!black} \bot}}
\centering
\scalebox{0.65}{
\input{img/BS_trsd.tikz}
}
\vspace*{-1cm}
\caption{Symbolic transducer model of the BS discrimination algorithm. Hold states are represented with dashed borders. All states but the hold states are final (double bordered). Boolean values tell when therapy ($\thrp$) or no therapy ($\nthrp$) is given.}\label{fig:BS_SFT}
\end{figure}
